Centralized vs. Decentralized Multi-Agent Reinforcement Learning for Enhanced Control of Electric Vehicle Charging Networks

The widespread adoption of electric vehicles (EVs) poses several challenges to power distribution networks and smart grid infrastructure due to the possibility of significantly increasing electricity demands, especially during peak hours. Furthermore, when EVs participate in demand-side management programs, charging expenses can be reduced by using optimal charging control policies that fully utilize real-time pricing schemes. However, devising optimal charging methods and control strategies for EVs is challenging due to various stochastic and uncertain environmental factors. Currently, most EV charging controllers operate based on a centralized model. In this paper, we introduce a novel approach for distributed and cooperative charging strategy using a Multi-Agent Reinforcement Learning (MARL) framework. Our method is built upon the Deep Deterministic Policy Gradient (DDPG) algorithm for a group of EVs in a residential community, where all EVs are connected to a shared transformer. This method, referred to as CTDE-DDPG, adopts a Centralized Training Decentralized Execution (CTDE) approach to establish cooperation between agents during the training phase, while ensuring a distributed and privacy-preserving operation during execution. We theoretically examine the performance of centralized and decentralized critics for the DDPG-based MARL implementation and demonstrate their trade-offs. Furthermore, we numerically explore the efficiency, scalability, and performance of centralized and decentralized critics. Our theoretical and numerical results indicate that, despite higher policy gradient variances and training complexity, the CTDE-DDPG framework significantly improves charging efficiency by reducing total variation by approximately %36 and charging cost by around %9.1 on average...

==> Chapters/Introduction_V1.tex <==
\section{Introduction}
\IEEEPARstart{T}{he} fundamental challenge of power grid management is the power balancing, i.e.,  ensuring that electric power generation closely matches the instantaneous variable load demand over the course of a day. Electric power demand is lowest in the morning, increases in the afternoon hours, and peaks in the evening. To meet the demand, system operators constantly dispatch a centrally-controlled fleet of generators with different operating costs during a 24-hour cycle. The off-peak hours are typically covered by baseline generators, which are relatively less costly to operate, while faster and more expensive generation facilities are used for load following and ramping during peak hours.  
Therefore, the price of electricity is not constant during the day, rather, it is considerably more expensive during peak hours and grid-regulating events. Demand-side management (DSM) is a strategy employed by grid operators to encourage consumers to shift their usage to non-peak hours or reduce overall consumption. With new emerging electricity loads, such as electric vehicle (EV) systems, DSM becomes even more critical. For example,  the widespread adoption of EVs could pose significant challenges, such as increasing energy demand during peak hours. To address this challenge, effective management and coordination of EV charging and discharging behavior are essential to achieve two specific goals: (i) minimize charging costs for EV owners and meet their battery energy requirements~\cite{al2019review, abdullah2021reinforcement}, (ii) balance charging demand and prevent transformer overload during peak hours~\cite{nimalsiri2019survey}. To achieve these goals, designing efficient scheduling algorithms for  EV charging is of paramount importance.   
% We specifically tackle the \textbf{scalability and non-stationarity} challenges that arise as the number of agents increases for such applications.}
% }

{
Yet, designing an optimal charging strategy for a network of EVs is a complex task due to several factors: (i) uncertainty in dynamic electricity prices during the day, (ii) uncertainty in the behavior of EV owners as a function of their arrival and departure times, charging level preference, and duration of charging, (iii) congestion management and transformer overload due to the physical constraints of the underlying smart grid network. In fact, simultaneous charging EVs have the potential to overwhelm the transformers connected to the network.
In this case, it is desirable to develop \emph{distributed coordination and cooperation mechanisms} between EVs in order to react to real-time grid conditions, while ensuring the highest quality of charging for EV owners in terms of charging experience (cost, duration, etc.). }


{Model-based approaches such as binary optimization~\cite{sun2016optimal}, mixed-integer linear programming~\cite{paterakis2016coordinated}, robust optimization~\cite{ortega2014optimal}, stochastic optimization~\cite{wu2017two}, model predictive control~\cite{zheng2018online}, and dynamic programming~\cite{xu2016dynamic} have been used for EV charging control and optimal scheduling. 
In these approaches, the scheduling of EV charging is typically framed as an optimization control problem. Despite the promising results achieved in model-based approaches, they require an accurate system model that is typically unavailable, especially under uncertain conditions due to dynamic pricing and the behaviors of EV owners.}
% task within a distributed grid hosting numerous EVs. Additionally, the presence of uncertainties arising from real-time pricing and the behaviors of EV owners introduces further complexities to the model-based control of coordinated EV charging networks.}




{In contrast, model-free approaches offer an alternative that does not require an accurate model or prior knowledge of the environment.  Among these approaches, Deep Reinforcement Learning (DRL) stands out as a powerful technique for addressing sequential decision-making problems. Previous studies ~\cite{wen2015optimal,chics2016reinforcement,wan2018model,zhang2020cddpg} have utilized single-agent DRL techniques like Deep Deterministic Policy Gradient (DDPG) and Soft-Actor-Critic (SAC) for an individual EV or a group of EVs networks~\cite{jin2020optimal}.
These studies operate under the assumption of full observability, meaning that the DRL agent has access to the local information of the EVs such as battery level and arrival/departure time of the EV to the charging station. However, EV owners may not be willing to share this private information. To address this issue, Multi-Agent RL (MARL) can be used for distributed and decentralized control within EV networks\cite{da2019coordination,chu2022multiagent,zhang2022federated,zhang2023cooperative,yan2022cooperative}, in which each EV charger is equipped with an RL agent that operates based on local information, without a need to collect private information from other EV chargers/owners. }


% In this paper, we formulate the decentralized charging control of networked EVs as a Decentralized Partially Observable Markov Decision Process (Dec-POMDP), and implement MARL agents on top of a residential EV network. Unlike previous works \blue{\cite{??}}, we depart from the assumption of sharing global or local information among agents during execution. The only global observation shared among agents in our framework is the electricity price, which is dynamically determined by the upstream grid. The single-agent version of DDPG consists of one actor and one critic network, thereby combining elements of both policy-based methods (actors) and value-based methods (critics) to improve the stability and efficiency of reinforcement learning. In this case, the actor is responsible for selecting actions based on the current policy, while the critic evaluates the actions taken by the actor by estimating the value of states or state-action pairs. Now, in order to extend single-agent DDPG to multi-agent scenarios, we can consider two variations: \emph{decentralized critic  vs. centralized critic.} 
\begin{figure}[t]
   \centering
    \includegraphics[scale=0.3800, trim = 0.4cm 1cm 0.41cm 0.2cm, clip]{figs/system_model.pdf}
    \caption{Electric vehicle charging network with a shared energy source.}
    \label{System Model}
    \vspace{-.1in}
\end{figure}

In this paper, we formulate the decentralized charging control of networked EVs as a Decentralized Partially Observable Markov Decision Process (Dec-POMDP), and implement MARL agents on top of a residential EV network. Unlike previous works \cite{yan2022cooperative}, we depart from the assumption of sharing global or local information among agents during execution. The only global observation shared among agents in our framework is the electricity price, which is dynamically determined by the upstream grid. In our framework, each agent is structured with a DDPG setup, comprising an actor and a critic network. The actor's role is to choose actions according to the current policy, while the critic assesses these actions by estimating the value of states or state-action pairs. To execute our MARL control strategy, we explore and contrast two well-known MARL variations: decentralized critic versus centralized critic.

In a decentralized critic instance, each agent has its own critic network; therefore, each agent regards the other agents as part of the environment, effectively ignoring their policies. In this paradigm, agents undergo independent training without sharing information with other agents. We refer to this method as Independent-DDPG (I-DDDPG). It has been shown that the decentralized critic approach may lead to poor convergence due to the nonstationarity of the environment~\cite{lyu2021contrasting,kuba2021settling}.  In contrast, in a centralized critic scenario, a single critic network is shared among all agents during the training stage. In this case, due to a shared critic network, the cooperation between agents is enhanced, which in turn stabilizes the training process~\cite{lowe2017multi}. This leads to a centralized training-decentralized execution (CTDE) architecture that enables agents to use a centralized critic during training to utilize additional information (from other agents) exclusively for training purposes only. Once training is completed, only local actors are engaged during the execution phase, thus maintaining a decentralized operation during execution without the need to share any information. Learning from the centralized critic helps in tackling the nonstationarity issue of I-DDPG~\cite{lyu2021contrasting,kuba2021settling}. Additionally, we offer a theoretical analysis comparing I-DDPG and CTDE-DDPG for an EV charging network. Our demonstration highlights that although the CTDE version suffers from scalability issues and high variance, it surpasses the I-DDPG in terms of promoting efficient charging behavior and minimizing costs. This comparative study sheds light on the strengths and weaknesses of each approach, providing valuable insights for optimizing EV charging network management strategies. In summary, the main contributions of this paper are as follows: 
\begin{itemize}
    \item This paper introduces a cooperative MARL framework designed to address the EVs network charging problem. The problem is formulated as POMDP, and the mathematical formulation for decentralized control has been proposed.
    \item We leverage the benefits of CTDE framework to relax the assumption of observing the global network parameters and exchanging private information between agents.
    \item We theoretically demonstrate that opting for a centralized critic is not always the obvious choice and depends on the environment, as both CTDE-DDPG and I-DDPG approaches ultimately converge to the same policy on average.Additionally, a centralized critic offers greater variance, impacting learning stability and convergence speed negatively.
    \item We deploy both CTDE-DDPG and I-DDPG algorithms for our EV charging network problem, and our empirical results indicate that CTDE outperforms I-DDPG in this scenario. This is attributed to the significance of cooperative behavior in preventing transformer overload. Moreover, collaboration among agents can yield financial benefits for all participants in the network.
    \item We examine the performance of our CTDE-oriented framework for a EV network. We provide the simulation results for up-to 20 agents and investigate the scalability and robustness of the proposed framework. 
\end{itemize}

% We refer to this RL method as Multi-Agent Deep Deterministic Policy Gradient (MA-DDPG). 

% version of DDPG algorithm, there are two neural networks, namely actor and critic   paradigm, To model different variations of cooperation across multiple charging agents, we consider two variants of MARL paradigms:  
% As suggested in ~\cite{papoudakis2020comparative}, we consider decentralized critic as baseline. In the decentralized Critic referred to as , each agent treats the other agents as part of the environment, effectively ignoring their individual strategies.  

% However, considering this, the decentralized critic suffers from a drawback related to the  non-stationarity of the environment~\cite{lyu2021contrasting,kuba2021settling}, which provide poor convergence guarantee. We also consider decentralized critic since we have partially observability~\cite{papoudakis2020comparative}. 
% In the centralized critic paradigm, we introduce a state-of-the-art cooperative reinforcement learning technique called Multi-Agent Deep Deterministic Policy Gradient (MADDPG)~\cite{lowe2017multi} to foster cooperative behavior and stabilize the training process.



In our prior publication~\cite{10313469}, we compared the preliminary results of our CTDE-DDPG and I-DDPG frameworks for controlling an EV network within the energy grid. This paper serves as an extension of our previous work~\cite{10313469}, with a heightened emphasis on scalability, performance, and robustness of the algorithm. Specifically, we have expanded the scope by considering a scenario with 20 agents, each equipped with an EV charger—a configuration that closely mirrors real-world conditions, as it represents a reasonable number of EVs that can be connected to a shared transformer. The rest of this paper is organized as follows. Section~\ref{Section:RelatedWork} provides the most recent related work, with emphasis on RL-based frameworks. The network and system model formulation are described in Section~\ref{Section:SystemModel}. Section~\ref{Section:Principal} introduced the principal of the algorithm in details, and Section~\ref{Section:ControlStrategy} provides the MARL control strategy for the proposed EV network. Numerical results are presented in Section~\ref{Section:Results} and Section~\ref{Section:Conclusion} concludes the paper.

% \blue{What are our contributions?
% \begin{itemize}
%     \item Formulating the EV charging control as a MARL problem and developing two variations for the cooperation level between the agents. 
%     \item Investigating the performance of I-DDPG and CTDE-DDPG for EV charging control 
%     \item Contrasting the performance of these algorithms in terms of scalability, convergence, variance. 
% \end{itemize}
% }

==> Chapters/Related_work.tex <==
\section{Related Work}\label{Section:RelatedWork}
In recent years, researchers have devised various methodologies for coordinating the charging process of EVs to prevent transformer overload. One particularly notable solution that has seen widespread application is the Time-of-Use (ToU) pricing scheme. ToU pricing incentivizes EV owners to charge their vehicles during periods of low demand, typically referred to as off-peak hours, when electricity prices are more economical. For instance, Said and Mouftah, as detailed in~\cite{8910498}, introduced a peak load management model for an EV fleet, grounded in queuing theory within the ToU pricing framework. In~\cite{8345660}, the authors presented a distributed hierarchical coordination framework for regulating active and reactive power dispatch for a multitude of dispersed EVs, incorporating a predefined 15-minute interval ToU pricing scheme. Moreover, in~\cite{9672089}, the authors proposed a cooperative hierarchical multi-agent system for scheduling EV charging, employing a two-level optimization approach under the influence of the ToU pricing scheme.

A growing body of research has looked into using model-free reinforcement learning (RL) techniques to tackle problems related to EV charging and scheduling. For instance, in~\cite{wen2015optimal}, the EV charging problem was treated as a Markov Decision Process (MDP), and Q-learning with a lookup table was used to find the best charging strategy. In another study~\cite{chics2016reinforcement} in 2017, researchers introduced a method to reduce the long-term charging costs of individual EVs by predicting electricity prices using a Bayesian neural network. Similarly, in~\cite{wan2018model}, the authors employed two networks to extract useful features from electricity prices and approximate the optimal charging/discharging power for each EV.

Inspired by these works, Zhang et al.\cite{zhang2020cddpg} leveraged a DDPG architecture for controlling individual EV charging. They used a Long Short-Term Memory (LSTM) network to capture past energy price data. In a related study\cite{jin2020optimal}, researchers investigated the scheduling of large-scale EV charging in a power distribution network under varying renewable energy generation and electricity prices, utilizing the Soft Actor-Critic (SAC) algorithm.


The mentioned single-agent methods assume full environment visibility and train a single agent to control individual or groups of EVs centrally. However, this setup raises privacy and scalability issues. To address this, Multi-Agent Reinforcement Learning (MARL) has emerged as a solution. MARL has found applications in various areas like Volt-VAR control in distribution networks~\cite{gao2021consensus}, microgrid energy management~\cite{fang2021multi}, and traffic flow control~\cite{zeynivand2022traffic}.

In the context of EV networks, researchers have proposed multi-agent approaches to minimize energy costs and prevent transformer overloads during charging phase~\cite{da2019coordination}. Some studies, such as Chu et al.\cite{chu2022multiagent} and Zhang et al.\cite{zhang2022federated}, employ federated reinforcement learning for distributed problem-solving. Zhang et al.\cite{zhang2023cooperative} explored collaborative EV charging control based on DDQN for an EV station. A recent work by Yan et al.\cite{yan2022cooperative} introduced a cooperative MARL framework for residential EV charging. They used a neural network to approximate agent behaviors and employed the soft-actor-critic method. Notably, our approach relaxes the assumption that each EV can observe the entire network demand at any given moment, unlike the method proposed in~\cite{yan2022cooperative}.


% In this paper, we take one step further and deploy a multi-agent reinforcement learning paradigm as a reasonable solution. Decentralized critic has always been a primary option for MARL problems. But recent deep MARL works often use the CTDE training paradigm~\ref{XXX}. The pioneer of MADDPG in~\cite{lowe2017multi} mentions that providing more information to critic ease learning and make the learning of coordinated behavior easier. Following their work, other works authenticate this viewpoint in terms of better training speed, less variance and better robustness. However, the author in~\cite{lyu2021contrasting} proposed an opposite viewpoint. They provided a theoretical analysis comparing centralized and decentralized critic and implemented it over a wide range of popular domains. Their work shows that the decentralized critic often outperform the centralized critic. 

The CTDE multi-agent reinforcement learning paradigm has gained significant prominence in recent research endeavors. Among the various centralized critic paradigms employed, Multi-Agent Deep Deterministic Policy Gradient(MA-DDPG), Counterfactual Multi-Agent Policy Gradients(COMA), and Multi-Agent Proximal Policy Optimization(MAPPO) have emerged as the most renowned and widely-applied algorithms. COMA excels in addressing credit assignment problems, making it a suitable choice for scenarios where attributing outcomes to specific agent actions is challenging. On the other hand, MAPPO is recognized for its online policy framework, known for its remarkable sample efficiency. It distinguishes itself as a more versatile solution, capable of accommodating both continuous and discrete action space environments.

The primary focus of this paper centers on the control of EV network charging, emphasizing the coordination of participants' charging decisions. Within this context, MA-DDPG, introduced in~\cite{lowe2017multi}, holds prominence as an off-policy MARL framework that is particularly well-suited for environments characterized by continuous action spaces. It excels in addressing cooperative-centric problems, making it a suitable choice for applications where agents need to coordinate their actions effectively. 

In recent years, centralized critic methods, despite their convergence challenges, have emerged as the predominant choice for multi-agent RL settings. Nevertheless, the ongoing debate regarding the merits of centralized versus decentralized approaches, and the determination of the superior method, continues to be an active area in the literature. In an analytical exploration, the research presented in~\cite{lyu2021contrasting} offers a theoretical analysis of the advantages and disadvantages associated with centralized and decentralized critics in multi-agent RL. Their findings reveal that there is no universally optimal solution applicable to all MARL scenarios, and the choice is heavily contingent on the specific characteristics of the environment.

This paper extends the discourse by addressing an EV network charging control problem as a practical real-world application. Through our investigation, we demonstrate that, while both centralized and decentralized critics deliver satisfactory performance, the centralized critic outperforms the decentralized critic in terms of promoting cooperation within the system.
